Understanding the Performance Horizon of the Latest ML Workloads with NonGEMM Workloads

Among ML operators today, GEneralMatrix Multiplication (GEMM)-based operators are known to be key operators that build the main backbone of ML models. As their computational overhead dominates the overall execution time (e.g., 42.8% - 96.6% in our results), GEMM operators have been the prime optimization targets for fast ML inference. This led to advanced GPUs and accelerators available today, which provided significant boost in the GEMM performance compared to CPUs, aligned with the lesson from Amdahl's law. However, accelerating GEMM has significantly shifted the Amdahl's law's landscape for ML inference; due to the decreased GEMM execution time, the relative execution time of non-GEMM operators is now significant. Although the importance of non-GEMM performance is increasing, we have little knowledge about the non-GEMM performance horizon in the latest hardware platforms and models. Therefore, to guide non-GEMM-oriented optimizations, we conduct a thorough performance analysis of 17 widely adopted ML models in Hugging Face and Torchvision on workstation and data center platforms with/without GPUs. We discover that non-GEMM performance bottleneck is a considerable issue across all the platforms and models, accounting for 11.3% to 73.6% of total latency, on average. The challenge significantly aggravates when we apply quantization, which is a common model compression technique, due to the boosted GEMM performance and extra non-GEMM operators for dequantization and requantization. To provide insights into non-GEMM optimization targets, we demystify the most dominant non-GEMM operators for each model and deployment software. We also show that widely adopted optimizations such as operator fusion do not completely address the non-GEMM performance bottleneck, where non-GEMM operators still account for 15% to 48% of total latency.

==> Backup/05_CaseStudies.tex <==

\section{Case Studies}
\label{sec:case_studies}

%
We perform a thorough performance analysis of models in \autoref{tab:modeltable} on multiple hardware platforms listed in ~\autoref{tab:experiment_settings}.
%
The evaluated hardware platforms span from mobile to data center-class CPUs and GPUs.
%
We employ PyTorch, ONNX runtime, and TensorRT as deployment flows to investigate their impact on the performance horizon.
%

Using the aforementioned workload, hardware platforms, and deployment flow, we characterize the GEMM/non-GEMM performance for each model in \bench and investigate the impact of the hardware platform and deployment flow.
%
In addition, we also investigate the impact of widely adopted optimizations (operator fusion and quantization) and show that the non-GEMM performance is an issue even after applying common optimizations.

\input{Tables/tab_experiment_settings}
% \input{Tables/tab_alias}%

\subsection{Non-GEMM Performance Characterization Results}
\label{sub:task_dom}

%We discuss how non-GEMM operator's contribution to the end-to-end inference latency changes depending on task domains and discuss key non-GEMM operators in each domain.

We present the characterization results on datacenter and workstation platforms (Platforms A and B in~\autoref{tab:experiment_settings}) in \autoref{fig:server_op_breakdown}.
%
We focus on those two platforms since large language models do not fit into the mobile devices.
%
As expected, the relative contribution of non-GEMM operators to the end-to-end latency significantly increases after GPU acceleration, on average, from \TODO{XX\%} to \TODO{YY\%}. 
%
However, we observe each model show different trends, mainly affected by the non-GEMM operator types and the number of GEMM and non-GEMM operators in the original model. 
%
We summarize the most time-consuming non-GEMM operators in~\autoref{tab:expensive_ops} from the datacenter class platform (Platform A), which shows the diversity of the dominating non-GEMM operators in each model.
%
We highlight some notable models and delve into the details of their non-GEMM performance.

\betterparagraph{Swin Transformer} For every Swin Transformer variant(Sw-t, Sw-s, and Sw-b), the memory operator group is the most latency-dominant non-GEMM operator group, which accounts for 32\% of the total inference latency, on average, on data center platform with GPU acceleration.
%  
Those memory operators originate from the Swin Transformer's unique window shape (cross-shaped)~\cite{liu2021swin}, which is not well-aligned with memory layout of tensor data organized in dimension orders. 
%
%Such memory operators account for  For example, Swin-b spends around 34\% of the inference time computing 1000 memory operators (~60\% of the total number of operators). 

\betterparagraph{DETR}
DETR computed non-GEMM operators for 66\% of the inference time on the data center GPU.
%
Normalization operators took a significant 35\% and 32\% of the execution time of DETR as indicated in \autoref{fig:server_op_breakdown} and in \autoref{fig:workstation_op_breakdown}.
% 
DETR uses normalization functions with custom implementations that do not leverage available library normalization kernels. 
This leads to additional overheads to execute the normalization function on GPU due to the accumulated overheads from running multiple kernels for a single operator. 




%Swin transformers divide input images into windows of patches. The shape of the windows is not static across model layers. 
%
%The windows get shifted to yield a different shape every layer. 
%  
%Achieving this functionality requires a significant amount of memory operators and tensor reshaping. 
%  
%For example, Swin-b spends around 34\% of the inference time computing 1000 memory operators (~60\% of the total number of operators). 


%we observe a clear change in relative break-down latency across operators when using a GPU.
%
%For example, the non-GEMM operations are minor before GPU acceleration, but they become dominant with a GPU, and account for around 41\% of the total execution time, on average.
%
%We observe similar patterns for most the other cases: non-GEMM operators become significant or considerable after GPU acceleration.

\betterparagraph{Image Classification} We observe 

For the three Swin transformer variants, memory operators are the most latency dominant non-GEMM operator, and account for 32\% of the total inference time when running on datacenter GPU.  
%  
Swin transformers divide input images into windows of patches. The shape of the windows is not static across model layers. 
%  
The windows get shifted to yield a different shape every layer. 
%  
Achieving this functionality requires a significant amount of memory operators and tensor reshaping. 
%  
For example, Swin-b spends around 34\% of the inference time computing 1000 memory operators (~60\% of the total number of operators). 
%  

For ViT models, the relative execution time of Non-GEMM operators for running ViT-b16, ViT-l16, and ViT-h14 increases from 10\%, 9.5\%, and 8.5\% when running on a CPU only platform to 29\%, 28\% and 27\%, respectively, on the GPU as shown in ~\autoref{fig:server_op_breakdown}.
%
The non-GEMM operators with the highest inference latency contribution in the ViT models are normalization with 12.66\%, followed by element-wise Arithmetic. 

For both Swin and ViT, ~\autoref{fig:workstation_op_breakdown} shows similar trends when running on the workstation GPU system. 
% 
As shown in ~\autoref{tab:expensive_ops}, memory and normalization are the non-GEMM operators with the highest contribution to the inference latency depends on the model architecture in classification models. 
%
Based on the collected data, image classification models require 38.5\% of  execution time on non-GEMM operators on GPU systems, on average, across all the evaluated models.
% 
\subsubsection{Object Detection}
\label{subsub:case-det}
%
Non-GEMM operator's latency is also noticeable for object detection models running on a GPU.
%
On the data center, non-GEMM operators dominated the execution time of FasterRCNN by consuming 67\% of the total inference time when we accelerate the workload compared to 53\% when running the CPU only (\autoref{fig:server_op_breakdown}). 
% 
FasterRCNN and MaskRCNN showed a similar behavior after acceleration, with an average of 63\% of the time time spend on non-GEMM operators on datacenter and workstation GPU.
% 
DETR computed non-GEMM operators for 66\% of the inference time on the data center GPU.
%
Normalization operators took a significant 35\% and 32\% of the execution time of DETR as indicated in \autoref{fig:server_op_breakdown} and in \autoref{fig:workstation_op_breakdown}.
% 
DETR uses normalization functions with custom implementations that do not leverage available library normalization kernels. 
This leads to additional overheads to execute the normalization function on GPU due to the accumulated overheads from running multiple kernels for a single operator. 

% 
Overall, the evaluation data shows that detection models get dominated by non-GEMM operators (66\%) when executing the workloads on a GPU system. 
% 
\subsubsection{Segmentation} 
\label{subsub:case-seg}
% \insertFigure {segmentation_breakdown}{The breakdown between GEMM and non-GEMM operators for segmentation workloads.}
For segmentation models, the non-GEMM operators account for 42.5\% of the execution time when running the inference on the CPU on average. 
% 
Upon running the model on the GPU, this number slightly increases to 53\%. 
%
For the SegFormer model, Normalization operators are the most expensive (15\% of the execution time), while Memory operators dominate the non-GEMM operators of Maskformer (24\%) as shown in~\autoref{fig:server_op_breakdown}.
% 

% 
\subsubsection{Language Models}
\label{subsub:language_models}
~\autoref{fig:server_op_breakdown} and~\autoref{fig:workstation_op_breakdown} show that non-GEMM operator latency becomes more considerable after running the inference on a GPU system. 
%  
On average, the non-GEMM contribution to the total inference latency increasd by XX$\times$ on average for language models. 
%  
For GPT2 models, activation operators have the highest non-GEMM latency contribution accounting for 30\% and 25\% of the inference runtime on the datacenter and workstation GPUs respectively. 
%  
Llama2 also showed a considerable non-GEMM latency contribution that almost doubled after GPU acceleration to become around 30\%. 
% 
Normalization operators are the slowest non-GEMM operators in Llama2, running for 15\% of the total execution time as seen in~\autoref{fig:llm_onnx_vs_eager}. 
\input{Tables/tab_expensive_ops_new}
% 
\insertWideFigure {server_op_breakdown}{Breaking down the execution time of models running on the Data Center (CPU only) and (CPU + GPU) configurations across operator groups. }
% 
% \insertWideFigure{workstation_op_breakdown}{Breaking down the execution time of models running on the Workstation (CPU only) and (CPU + GPU) configurations across operator groups. }
% 
\autoref{fig:llm_onnx_vs_eager} (a) suggests that the bottleneck are activation, arithmetic, and memory operators.
% 
GPT2 models implement their own GELU activation in the Hugging Face library which does not have a direct mapping to a GELU GPU kernel when running in PyTorch. 
% 
This leads to additional overheads due to running multiple kernels to compute the activation. 
% 
Similarly, Llama2 uses a normalization function that does not map to a single GPU kernel in PyTorch which leads to similar overheads that increase the latency of the non-GEMM operators. 
%


\subsection{Impact of Deployment Flow on Non-GEMM}
\label{subsec:deployment_flow_effect}
%
Deployment flows such as ONNX runtime~\cite{onnxruntime} and TensorRT~\cite{tensorrt} facilitate the model service process by applying various optimizations to each model and executing inferences with such optimizations.
%
The optimizations include the computational graph level optimizations (e.g., operator fusion) and backend assignment (e.g., utilizing Tensor Core in Nvidia GPUs).
%


%Running in PyTorch, Non-GEMM operators occupy large proportions of the execution time for various applications running on the GPUs , as summarized in~\autoref{tab:expensive_ops}. 
% 
%Nevertheless, deployment frameworks (e.g. \cite{onnxruntime, chen2018tvm}) are typically used to improve performance.
% 
%They apply transforms at the computational graph level and leverage accelerators (if available) to optimize the inference runs. 
% 
To understand the effect of deployment frameworks on the operator performance, we evaluate our models with ONNX Runtime (ORT).
% how deployment frameworks affect inference performance distribution across operators, we evaluate our models with ONNX Runtime (ORT).
% 
ORT is a cross platform ML framework that accelerates ML model inferencing~\cite{onnxruntime}. 
% 
It leverages hardware accelerators (e.g. GPUs) and operator graph level optimizations to improve the performance of ML models.
%
We run selected models with the CUDA execution provider and observe the following results:


%% Non-GEMM follow the same trend with ORT with SOTA models
Non-GEMM operators account for a significantly larger proportion of the total execution latency (\autoref{fig:onnx_hw_comparison}) when running on different grade GPUs.
% 
This is aligned with the trend observed with the PyTorch execution on GPU. 
% 
On average, the time spend on non-GEMM operators increases from  52.6\% to a 80.75\% after deploying the models on GPU with the ORT cuda execution provider.
%  
% Compare the average execution time proportion of GEMM and Non-GEMM between Pytorch and ORT and 
% 
%% The latency expensive operators on ORT are not the same as Torch

Memory operators almost dominate the execution time in three application domains, classification, language models and segmentation by occupying 94\%, 85\%, 45\% respectively.
% 
For instance, memory operators are the most latency expensive non-GEMM operators in GPT2-XLarge and Llama2-7b as they consume 76\% and 59\% of the total inference time respectively (\autoref{fig:llm_onnx_vs_eager}). 
%

One reason leading memory operators to dominate the inference latency is their high frequency, notably in the large language models.
%
They consist of 80\% and 62\% of the total operators in the GPT2-XLarge and Llama2-7b.
% 
Consequently, the cumulative latency to run these operators becomes the inference latency bottleneck. 
%
Another reason is the limitations in operator support for GPU deployment in ORT.
% 
Memory operators are a subset of non-GEMM operators that the cuda execution provider does not fully support, hence it assigns them to be computed on the CPU. 
%
In the case we hit an unsupported operator while executing on the GPU, the runtime falls back to CPU to carry the computation. 
% 
As a result, additional overheads to transfer the data between devices are added to the operators execution time that increases the latency of the fallen-back operators, which aggravates frequently used operators.
% 
\autoref{fig:llm_onnx_vs_eager} highlights the differences in operator latency distribution for GPT2-XLarge and Llama2-7b running in PyTorch eager mode and ORT.
% 
Despite dominating the execution time in ORT for the majority of the evaluated models, memory operators were not the main non-GEMM bottlenecks PyTorch. 
% 
% 
\textit{This indicates that the deployment flows have distinct effects on the execution of non-GEMM operators in an end to end inference.} 
%

In detection models, we notice a different trend than the remaining task domains. 
%  
The non-GEMM operator with the highest contribuion to the inference latency varies across platforms. 
% 
We notice arithmetic operators dominate 52\% of the execution when running on the mobile GPU platform, while memory operators consume 6\% of the execution time, becoming the main bottleneck on the datacenter platform. 
% 
The datacenter GPU speeds up arithmetic (the operator is NonZero, I included it under elmt-wise arithmetic) operators by 1.6$\times$. Running on the mobile GPU on the other hand, reduces the latency of these operators by a factor of 6.8$\times$, making them the major inference bottleneck on the mobile GPU. 
% 
This indicates that HW platform will affect the performance of non-GEMM operators.   
% 

\insertFigure{llm_onnx_vs_eager}{The impact of deployment software toolchain into the latency breakdown on language models. (a) PyTorch and (2) ONNX Runtime on a data center class GPU (A100).}

\insertFigure{onnx_hw_comparison}{\TODO{Add Workstation to the plot}The latency breakdown of the inference using ORT on two platform configurations: mobile and Data Center.}

\insertFigure{server_trt_cv} {The latency of non-GEMM operator in (a) Swin-b, (b) DETR, and (c) Segformer is still considerable despite applying operator fusion in TensorRT. The numbers at the top of each bar represent the latencies in milliseconds.}



% \insertFigure{server_trt_lm}{Non-GEMM operators contribution to end-to-end LLM inference latency is still considerable despite applying operator fusion.  For (a) GPT2-XL and (b) Llama2, non-GEMM latency increases with the sequence length when running in TensorRT.}







\subsection{Non-GEMM Performance with Operator Fusion}
\label{subsec:fusion}

% \TODO{Swin-b data in Fig.9 shows that even with optimizations applied to non-GEMM operators, non-gemm is still considerable}

% \TODO{Look at the swin-tiny TRT vs Pytorch gemm non gemm and speed up. We want to verify the claim that models like segformer and swin-tiny were dominated by non-compute operations}

% \TODO{Main point we are showing is the effect of the fusion, We can notice that normalization is fusion friendly, while other operators in the Segformer}
Operator fusion is a key optimization technique for accelerating inference workloads~\cite{dao2022flashattention, korch, symons2023streamfuse, niu2021dnnfusion, tensorrt, kao2023flat}. 
% 
Fusion combines multiple operators in a single kernel to reduce the number of costly kernel launches and minimize the number of redundant offchip memory accesses~\cite{niu2021dnnfusion}.
%input reads and intermediate tensor stores~\cite{niu2021dnnfusion}. 
% 
TensorRT~\cite{tensorrt} is a widely adopted inference framework  released by Nvidia that applies the operator fusion technique targeting GPUs.
% 
Operator fusion in TensorRT detects specific patterns (e.g., three consecutive element-wise operators~\cite{tensorrt}) in the operator graph and fuses nodes captured in the patterns to enhance inference performance by reducing redundant memory accesses around non-GEMM operators. 
% 
%Common fusion patterns include combining multiple element-wise non-GEMM operators or integrating non-GEMM operators with GEMM operators to alleviate latency bottlenecks.
% 
%Typically, operator fusion is applied to reduce non-GEMM operator bottlenecks when accelerating the inference on GPU. 
%  

% Although operator fusion is a technique typically applied to reduce bottlenecks of non-GEMM operators that get amplified by GEMM acceleration on GPU, we notice in~\autoref{fig:server_trt_cv} that fusion does not fully address non-GEMM operators bottlenecks for all models.
% 
% 

\betterparagraph{Impact of Operator Fusion} To understand the impact of operator fusion on non-GEMM performance horizon, we conduct a case study on four models, which compares the TensorRT (with fusion) and PyTorch (without fusion).
%
We present the results in~\autoref{fig:server_trt_cv}, which shows the inference latency breakdown between GEMM and non-GEMM operators.
%
We notice that fusion does not completely address the non-GEMM bottleneck in Swin-b model. 
%
For example, the percentage of non-GEMM operators in the total latency changes from 56.2\% to 32.2\%, on average, after operator fusion by TensorRT.
%
The reduction in the percentage is based on the improvement of non-GEMM performance via operator fusion, which reduces 88.6\% of latency after fusion, as summarized in~\autoref{tab:fusion_rate}.
%
However, the non-GEMM operators still account for 32.2\% of total latency, which is considerable.
%
This shows that operator fusion cannot eliminate the non-GEMM performance challenge and motivates further studies toward non-GEMM performance.

%before applying fusion, non-GEMM operators dominate Swin-b inference latency, accounting for 58\% of the total.


%After Applying operator fusion with TensorRT speeds up the Swin-b non-GEMM latency by 8.84$\times$ as indicated in~\autoref{tab:fusion_rate}. 
%  
%However, non-GEMM operators still contribute a considerable 39\% of the total inference latency. 
% 
%\textit{This indicates that fusion does not fully mitigate the non-GEMM bottleneck}.
% 

\betterparagraph{Factors Affecting the Effectiveness of Fusion} Although most results indicate considerable impact of non-GEMM even after operator fusion, we observe operator fusion on DETR model is exceptionally effective.
%
Therefore, we conduct a deep-dive study, investigating the percentage of fused non-GEMM operators (i.e., fusion rate) and performance improvements after fusion, as listed in~\autoref{tab:fusion_rate}.
%
We observe the strong non-GEMM performance improvements for DETR originates from high fusion rate of 30\%, which led to 13.5$\times$ non-GEMM speedup.
%
This leads to the large percentage reduction of non-GEMM in the total latency, from 67\% to 18.5\%, on average.
%

However, the fusion rate is not the only factor that determines the non-GEMM speedup.
%
For example, DETR and Segformer have similar fusion rates (30\% andn 27\%, respectively), but the amount of non-GEMM performance improvements are significantly different: 13.5$\times$ and 2.39$\times$, respectively. 
%
We analyze the execution trace and find that batch normalization is the main source of the differences.
%
The main difference is the fusion pattern: most batch normalization operators (\TODO{100\%} of total) in DETR were fused with GEMM-operators (CONV+BN+ReLu pattern) while those in Segformer were fused with other non-GEMM operators (\TODO{99.9\%} of total). 
%
The results indicate that the effectiveness of operator fusion relies on not only the overall fusion rate but also the fusion patterns.
%DETR: 84 ops 
%SegFormer: 31 ops 
%
Note that the effective fusion pattern in DETR originates from the convolutional neural network used as backbone: as Transformer-based models are trending to be state-of-the-art, we cannot expect DETR-like improvements in general.
%
Our observation confirms that the operator fusion cannot fully address the non-GEMM performance challenge, even if it can be very effective on some patterns.

\begin{comment}
~\autoref{tab:fusion_rate} indicates that TensorRT fuses 30\% of non-GEMM operators in DETR.
% 
The applied fusion speeds up non-GEMM execution by 13.5$\times$, and results in a significant decrease in the portion of inference time spent on non-GEMM operators in DETR from 67\% in PyTorch (no fusion applied) to 18.5\% on average as presented in~\autoref{fig:server_trt_cv}
% 
For Segformer, the non-GEMM fusion rate is 27\%.
%  
At a similar fusion rate to DETR, the contribution of non-GEMM operators to inference latency does not change after operator fusion was applied.
% 
Non-GEMM operators account for 41\% of the Segformer latency, despite a 2.4$\times$ non-GEMM latency speedup observed in~\autoref{tab:fusion_rate}. 
%
Although the fusion rates of DETR and Segformer are similar (30\% and 27\%), nevertheless the reduction in non-GEMM latency contribution is significantly different, which suggests that the non-GEMM fusion rate is not solely the reason for reduced non-GEMM bottleneck.
%  
TensorRT fusion heavily improves the performance of non-GEMM operators in DETR achieving a non-GEMM speedup of 14$\times$. 
TensorRT also speedup GEMM operators in DETR by 1.66$\times$. Because the non-GEMM speedup was significantly larger for DETR, it reflects as a decrease in the proportion of non-GEMM latency. 
% 
For the segformer, TensorRT speeds up GEMM and non-GEMM operators by 3.4$\times$ and 2.9$\times$ respectively. 
% 
The non-GEMM speed-up is slightly smaller than the GEMM speed-up which reflects in the unchanged latency distribution between GEMM and non-GEMM for Segformer showed in~\autoref{fig:server_trt_cv}. 
 
% Key Takeaways
% Non-GEMM Fusion does not fully mitigate the non-GEMM bottleneck. This is empirically shown by the swin data. 
% Non-GEMM Fusion rate does not solely affect the contribution of non-GEMM ops to the inference latency --> Why? tab:fusion_rate indicates that DETR and Segformer have fusion rates ~ 30%, DETR non-gemm pct significantly decreased while segformer it was not the case. Swin has a low fusion rate, significant decrease in the non-gemm latency.
%
\end{comment}

\subsection{Non-GEMM Performance with Quantization}
\label{subsec:quantization}

Quantization refers to the model optimization technique, which reduces the bit precision of model weights and/or activations to enhance the computational performance and efficiency of DNN inference.
%
Quantization is a widely-adopted technique~\cite{jacob2018quantization, nagel2021whitequant} including heavy models like LLMs~\cite{frantar2022gptq, lin2024awq, xiao2023smoothquant, llm.int8}.
%
For example, LLM.int8()~\cite{llm.int8} introduced an 8-bit - 16-bit mixed precision quantization scheme for LLMs.
%
LLM.int8() is a state-of-the-art quantization method, which quantizes more than 99\% of the linear layers in OPT LLM to an 8-bit precision.
%
Therefore, we adopt LLM.int8() and characterize GEMM and non-GEMM performance to understand the impact of quantization on the non-GEMM operator performance problem.

% 
%  
%To understand the implication of the mixed precision quantization on the operator performance latency of LLMs, we compare the inference latency Llama3-8B running in full precision mode (16-bit) and in quantized mode with LLM.int8() quantization applied.


%is a widely-adopted optimization technique applied to enhance the computational performance and efficiency of DNN inference. 
%
% reduces the bit precision of model weights and/or activations to improve latency and energy performance~\cite{jacob2018quantization, nagel2021whitequant}. 
%
%Quantization is also heavily applied to very large models, especially LLMs like Llama3~\cite{dubey2024llama3}, to reduce their memory footprint as well.~\cite{frantar2022gptq, lin2024awq, xiao2023smoothquant, llm.int8}. 
% 
%~\cite{llm.int8} introduced LLM.int8() an 8-bit - 16-bit mixed precision quantization scheme for LLMs. 
%  
%LLM.int8() quantizes more than 99\% of the linear layers in the transformer model (~\autoref{fig:models_architecture} to an 8-bit precision.
% 
%The GEMM operators of the quantized linear layers are computed using the 8-bit precision, while the remaining operators are computed using the 16-bit precision. 
%  
%To understand the implication of the mixed precision quantization on the operator performance latency of LLMs, we compare the inference latency Llama3-8B running in full precision mode (16-bit) and in quantized mode with LLM.int8() quantization applied. 
%  

We conduct a case study on quantization using LLM.int8() on Llama3 LLM on the datacenter platform with GPU acceleration and present the results in~\autoref{fig:server_quantization}.
%
In the results, we observe that non-GEMM operators dominate the latency after quantization, changing from 29.3\% to 76.7\%, on average.
%
Such a significant shift in the latency distribution is mainly based on the GEMM performance improvements from 8-bit arithmetic, which reduced the latency by 38.2\%, on average.
%
However, based on our analysis on the execution traces, non-GEMM performance aggravates because the 8-bit data need to be dequantized and re-quantized for non-GEMM operators, which requires 16-bit floating point arithmetic.
%
This led to 6510 additional non-GEMM operators into the computational graph, which led to a significant increase of the non-GEMM latency by 5.6$\times$ after quantization.
%q
Combined together, the overall percentage of non-GEMM operators in the total latency dominate after quantization, which makes non-GEMM operators as the major optimization target.

In the case study on Llama3 8B, we observe the element-wise arithmetic operators originate from dequantization/requantization (DQRQ) process dominate in the inference latency, which adds 20\% extra non-GEMM operators to the original computational graph. 
% 
Also, we observe longer sequence length leads to higher percentage in the element-wise arithmetic operators.
%
For example, as we increase the sequence length from 512 to 8192, the latency percentage of element-wise arithmetic operators increase from 31.8\% to 63.8\%.
%
As current trends in the LLMs are toward longer sequence lengths~\cite{dubey2024llama3, achiam2023gpt4}, the non-GEMM performance issues in longer sequences originating from DQRQ costs will aggravate, which motivates efforts in non-GEMM performance optimization.


%We observe that element-wise arithmetic operators latency significantly increased by 23$\times$ in the quantized model, and the added operators incur an extra latency of 723 ms with a sequence length of 8192. 
% 
%This observation is consistent across various sequence lengths, and implies that \textit{mixed precision quantization of LLMs renders the non-GEMM bottleneck more significant}. 



%a direct byproduct of running 8-bit GEMM operators, that originally dominated 70\% of the execution time in the 16-bit precision inference. 
% 

%The GEMM operators of the quantized linear layers are computed using the 8-bit precision, while the remaining operators are computed using the 16-bit precision. 


%For input sequence of 8192, the latency to compute GEMM operators decreased by around 2$\times$ to become 504 ms in the quantized inference.
% 
%On the other hand the non-GEMM latency increased by 5.6$\times$ 304 ms to 1700 ms after quantization.
% 
%Since 8-bit computation is only supported for linear GEMM layers, activations must be dequanztized and casted back to the original 16-bit precision to compute the non-GEMM operators. 
%  
%Therefore, 6510 additional non-GEMM operators are added per inference to support mixed precision, and the online quantization and dequantization process.
%  
%20\% of the additional non-GEMM operators are element-wise arithmetic operators. 
% 
%We observe that element-wise arithmetic operators latency significantly increased by 23$\times$ in the quantized model, and the added operators incur an extra latency of 723 ms with a sequence length of 8192. 
% 
%This observation is consistent across various sequence lengths, and implies that \textit{mixed precision quantization of LLMs renders the non-GEMM bottleneck more significant}. 

\insertFigure{server_quantization}{Non-GEMM operators latency contribution to the inference of a quantized Llama3 8B using 8 bit quantization~\cite{llm.int8}. The numbers at the top of each bar represent the latencies in milliseconds.} 

\input{Tables/tab_fusion_rate}

\subsection{Key Observations and Insights}
\label{subsec:observations}
%

We summarize our main observations and insights:
{
\begin{itemize}
%
{\item Accelerating GEMM operators using GPUs significantly shifts the performance horizon, which makes the non-GEMM operators main bottleneck of the systems: On average, non-GEMM breakdown increases from 27\% (CPU-only) to 55\% (CPU + GPU).}
%
{\item We observe the dominance of non-GEMM operators after GPU acceleration across all the platforms (mobile, workstation, and datacenter) and task domains, which indicates that the non-GEMM operator is emerging as a prime optimization target for every platform.
}
% 
{\item Existing optimizations such as operator fusion in deployment software do not fully address the non-GEMM operator performance challenge.}
%
{\item Depending on the optimizations applied in deployment software flows, the most time-consuming non-GEMM operators change.
%affects the most time-consuming non-GEMM operators: In ORT, memory operators dominate the execution time across all models (on average, 56\%), while PyTorch doesn't show clear patterns. 
}
%{\item Dominant non-GEMM operator class vary depending on the task category: In IC models, memory and  normalization operators dominate (on average, 38.6 and 13.8\% of the total execution time), while activation and normalization operators dominate in language models (29\% and 13.3\% for each, on average).
% 
%}
{\item Widely used model compression technique, quantization,  significantly aggravates the non-GEMM performance challenge because of the GEMM performance boost via quantization and non-GEMM operators requiring dequantization and requantization.
} 
{\item The profiling results indicate that the \textbf{non-GEMM operators are now the prime optimization target} after GEMM acceleration.
} 
\end{itemize}




==> Sections/08_Acknowledgments.tex <==
%\section*{Acknowledgments}
%HK: Shouldn't be included in the submission for review

==> Tables/tab_alias.tex <==
\begin{center}
\begin{table}
\caption{\bench Model aliases used in ~\autoref{fig:server_op_breakdown} and ~\autoref{fig:workstation_op_breakdown}.}
\scriptsize
\centering
\begin{tabular} {  | c | c | c |  } 

\hline
%
 \textbf{ Models }  & \textbf{Batch Size} & \textbf{ Model Alias }     \\
\hline
%
 \multirow{2}{*}{ViT Base 16} & 1 &  Vt-b b-1 \\ 
\cline{2-3} 
% 
 & 8 & Vt-b b-8  \\ 
\cline{1-3} 
%
\multirow{2}{*}{ViT large 16} & 1 & Vt-l b-1 \\ 
\cline{2-3}
%
& 8 &Vt-l b-8 \\ 
\cline{1-3}
% 
 \multirow{2}{*}{Swin Transformer tiny} & 1 & Sw-t b-1 \\ 
\cline{2-3}
%
& 8 & Sw-t b-8 \\ 
\cline {1-3}
% 
 \multirow{2}{*}{Swin Transformer small} & 1 & Sw-s b-1 \\ 
\cline{2-3}
% 
& 8 & Sw-s b-8  \\
\cline{1-3}
% 
 \multirow{2}{*}{Swin Transformer base} & 1 & Sw-b b-1 \\ 
\cline{2-3}
% 
& 8 & Sw-b b-8 \\
\hline
%
 \multirow{3}{*}{FasterRCNN} & 1 & FRCNN b-1 \\ 
\cline{2-3}
%
& 2 & FRCNN b-2 \\
\cline {2-3}
%
& 8 & FRCNN b-8 \\
\cline {1-3}
%
 \multirow{3}{*}{MaskRCNN} & 1 & MRCNN b-1 \\
\cline{2-3}
%
& 2 & MRCNN b-2 \\ 
\cline {2-3}
% 
& 8 & MRCNN b-8 \\ 
\cline {1-3}
% 
DETR & 2 & DETR b-2 \\ 
\hline 
%
 \multirow{2}{*}{GPT2} & 1 & gpt2 b-1\\
\cline{2-3}
%
& 64 & gpt2 b-64 \\ 
\cline {1-3}
%
 \multirow{2}{*}{GPT2 Large} & 1 & gpt2-L b-1 \\
\cline{2-3}
%
& 64 & gpt2-L b-64\\
\cline{1-3}
%
GPT2 X-Large & 1 & GPT2-XL b-1 \\
\cline{1-3}
%
 Llama2-7B & 1 & Llama2-7b b-1 \\
\cline {1-3}
%
\multirow{2}{*} {Bert} & 1 & bert b-1 \\
\cline {2-3}
%
& 64 & bert b-64 \\ 
\hline

\end{tabular}
\label{tab:alias}

\end{table}
\end{center}

==> Tables/tab_comparison_related_works.tex <==
\begin{table}
\caption{Comparing \bench with existing benchmarks: MLPerf~\cite{reddi2020mlperf}, LongTail Bench~\cite{longtailbench}, TorchBench~\cite{hao2023torchbench}, and \bench (This work).}
\scriptsize
\centering
\begin{tabular} {| c| c | c | c | c |  }
\hline

% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Benchmark  \\  
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Latency  \\ Breakdown 
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Popularity  \\ Driven 
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Micro-  \\Benchmark  
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Real Dataset  \\  Driven
% \end{tabular}} 
% & 
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Plug Model  \\ \& Profile\\ 
% \end{tabular}} 

% \\
% \hline 

% MLPerf ~\cite{reddi2020mlperf} &  & & & \checkmark & \\
% \hline

% LongTail ~\cite{longtailbench} & & & \checkmark & & \\ 
% \hline

% TorchBench ~\cite {hao2023torchbench} & &  \checkmark & & \checkmark & \\
% \hline 
% \bench & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
% \hline

%Benchmark & Latency Breakdown & Popularity Driven & Microbenchmark & Real dataset driven & Plug model and profile \\

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\textbf{Benchamrk}
\end{tabular}}
& 
\multirow{2}{*}{MLPerf}  
&  
\multirow{2}{*}{LongTailBench}
&
\multirow{2}{*}{TorchBench}
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
NonGEMMBench \\ (This work)
\end{tabular}}\\

&&&&\\


\hline 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Real Usage  \\ Driven 
\end{tabular}} 
& & &
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}
\\
&&&&
\\
\hline
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Non-GEMM \\ Focused  
\end{tabular}} 
&& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} \\

&&&&

\\
\hline
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Real Dataset  \\  Driven
\end{tabular}} 
& \multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}} &&&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}\\
&&&&
\\

\hline 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Plug Model  \\ \& Profile\\ 
\end{tabular}} 
& &&&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\checkmark
\end{tabular}}\\
&&&&\\
\hline
\end{tabular}
\label{tab:comparison_related_works}
\end{table}


==> Tables/tab_cpu_gpu_breakdown.tex <==
\begin{center}
\begin{table}
\caption{Breakdown of the execution time of operators for a selected models running on workstation platform. }
    \tiny 
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \multirow{2}{*}{Model}  & \multirow{2}{*}{Operator} & \multicolumn{3}{c|}{GPU + CPU} & CPU Only  \\ \cline{3-6}
        
        ~ & ~ & CPU Time  (us) & GPU time (us) & Total (us) & Total (us) \\ \hline
        
        \multirow{6}{*}{ViT-b16-batch-1} & GEMM & 16650.44227 & 2118.434442 & 18768.87671 & 42016.1409 \\ \cline{2-6}
        
        ~ & Non-GEMM  & 23768.86693 & 157.2054795 & 23926.07241 & 12514.59883 \\ \cline{2-6}
        
        ~ & Norm & 8699.684932 & 83.01369863 & 8782.69863 & 3347.78865 \\ \cline{2-6}
        
        ~ & Act & 3631.97456 & 25.23287671 & 3657.207436 & 1378.082192 \\ \cline{2-6}
        
        ~ & Arith & 8387.129159 & 44.95107632 & 8432.080235 & 4738.761252 \\ \cline{2-6}
        
        ~ & MemOp & 470.8493151 & 4.007827789 & 474.8571429 & 285.702544 \\ \hline
        
        \multirow{6}{*}{ViT-b16-batch-8} & GEMM & 16611.30159 & 8103.539683 & 24714.84127 & 244985.4127 \\ \cline{2-6}
        
        ~ & NonGEMM & 23351.06349 & 564.7619048 & 23915.8254 & 21208.52381 \\ \cline{2-6}
        
        ~ & Norm & 8555.555556 & 177.968254 & 8733.52381 & 4413.396825 \\ \cline{2-6}
        
        ~ & Act & 3583.174603 & 254.8571429 & 3838.031746 & 6105.063492 \\ \cline{2-6}
        
        ~ & Arith & 8232.777778 & 112.9365079 & 8345.714286 & 6596.142857 \\ \cline{2-6}
        
        ~ & MemOp & 533.984127 & 19 & 552.984127 & 353.984127 \\ \hline
        
        \multirow{7}{*}{Swin-small-batch-1} & GEMM & 39907.95499 & 2562.344423 & 42470.29941 & 62790.23092 \\ \cline{2-6}
        
        ~ & NonGEMM & 56343.23483 & 449.7377691 & 56792.9726 & 20763.49902 \\ \cline{2-6}
        
        ~ & Norm & 18493.18395 & 179.2328767 & 18672.41683 & 3384.569472 \\ \cline{2-6}
       
        ~ & Act & 7567.876712 & 50.15264188 & 7618.029354 & 2349.882583 \\ \cline{2-6}
        
        ~ & Arith & 15319.20548 & 55.95107632 & 15375.15656 & 6976.322896 \\ \cline{2-6}
        
        ~ & MemOp & 10762.09198 & 159.3933464 & 10921.48532 & 5138.966732 \\ \cline{2-6}
        
        ~ & Pooling & 404.1643836 & 5.007827789 & 409.1722114 & 179.6438356 \\ \hline
        
        \multirow{7}{*}{Swin-small-batch-8} & GEMM & 38748.79365 & 7742.52381 & 46491.31746 & 301921.3333 \\ \cline{2-6}
        
        ~ & NonGEMM & 54719.14286 & 1056.349206 & 55775.49206 & 35682.7619 \\ \cline{2-6}
        
        ~ & Norm & 18470.36508 & 453.6349206 & 18924 & 6848.746032 \\ \cline{2-6}
        
        ~ & Act & 7505.984127 & 220.9206349 & 7726.904762 & 8390.968254 \\ \cline{2-6}
        
        ~ & Arith & 15197.44444 & 194.5555556 & 15392 & 10655.71429 \\ \cline{2-6}
        
        ~ & MemOp & 10490.50794 & 182.1111111 & 10672.61905 & 6367.301587 \\ \cline{2-6}
        
        ~ & Pooling & 340.4444444 & 5.126984127 & 345.5714286 & 187.5714286 \\ \hline
        
        \multirow{7}{*}{GPT2-batch-1} & GEMM & 31184.20352 & 1224.491194 & 32408.69472 & 33756.36791 \\ \cline{2-6}
        
        ~ & NonGEMM & 98842.03131 & 433.5048924 & 99275.5362 & 35683.49511 \\ \cline{2-6}
        
        ~ & Norm & 8736.489237 & 78.7964775 & 8815.285714 & 1906.369863 \\ \cline{2-6}
        
        ~ & Act & 30429.26419 & 165.4657534 & 30594.72994 & 5303.311155 \\ \cline{2-6}
        
        ~ & Arith & 18503.88258 & 84.38551859 & 18588.2681 & 5178.23092 \\ \cline{2-6}
        
        ~ & MemOp & 24863.66928 & 66.57925636 & 24930.24853 & 10191.07632 \\ \cline{2-6}
        
        ~ & Softmax & 3940.872798 & 31.39921722 & 3972.272016 & 1072.44227 \\ \hline
        
        \multirow{7}{*}{GPT2-batch-16} & GEMM & 31957.41935 & 19423.06452 & 51380.48387 & 674009.7742 \\ \cline{2-6}
        
        ~ & NonGEMM & 97856.96774 & 17246.03226 & 115103 & 376959.0323 \\ \cline{2-6}
        
        ~ & Norm & 8719.193548 & 330.6774194 & 9049.870968 & 8241.451613 \\ \cline{2-6}
        
        ~ & Act & 30523.67742 & 10668.45161 & 41192.12903 & 207763.7097 \\ \cline{2-6}
        
        ~ & Arith & 18477.12903 & 3472.677419 & 21949.80645 & 71270 \\ \cline{2-6}
        
        ~ & MemOp & 24327.74194 & 1283.258065 & 25611 & 45067.12903 \\ \cline{2-6}
        
        ~ & Softmax & 3852.354839 & 1466.774194 & 5319.129032 & 31275.74194 \\ \hline
        
        \multirow{7}{*}{GPT2-Large-batch-1} & GEMM & 95700.28571 & 7637.911937 & 103338.1977 & 218225.3268 \\ \cline{2-6}
        
        ~ & NonGEMM & 302483.9648 & 1536.931507 & 304020.8963 & 132494.407 \\ \cline{2-6}
        
        ~ & Norm & 26186.90802 & 270.9549902 & 26457.86301 & 9476.976517 \\ \cline{2-6}
        
        ~ & Act & 92491.7319 & 628.0998043 & 93119.8317 & 25988.68297 \\ \cline{2-6}
        
        ~ & Arith & 57705.94521 & 303.6634051 & 58009.60861 & 25796.62622 \\ \cline{2-6}
        
        ~ & MemOp & 76773.90215 & 217.741683 & 76991.64384 & 34278.5362 \\ \cline{2-6}
        
        ~ & Softmax & 11540.80822 & 108.9471624 & 11649.75538 & 3886.178082 \\ \hline
        
        \multirow{7}{*}{GPT2-Large-batch-64} & GEMM & 101309.2258 & 139389.2581 & 240698.4839 & 5132246.935 \\ \cline{2-6}
        
        ~ & NonGEMM & 326921.6452 & 96818.35484 & 423740 & 1843876.968 \\ \cline{2-6}
        
        ~ & Norm & 26886.09677 & 1413.806452 & 28299.90323 & 44316.90323 \\ \cline{2-6}
        
        ~ & Act & 97057.64516 & 61441.77419 & 158499.4194 & 1043040.839 \\ \cline{2-6}
        
        ~ & Arith & 60932.19355 & 18790.06452 & 79722.25806 & 355737.3226 \\ \cline{2-6}
        
        ~ & MemOp & 86503.41935 & 6996.096774 & 93499.51613 & 201767.129 \\ \cline{2-6}
        
        ~ & Softmax & 12168.09677 & 8134.677419 & 20302.77419 & 156385.1613 \\ \hline
    
    \end{tabular}
    \label{tab:cpu_gpu_breakdown}    
\end{table}
\end{center}

==> Tables/tab_energy.tex <==
\begin{center}
\begin{table}
\caption{Most time-consuming non-GEMM operator groups for selected Models (Platform A, with GPU acceleration, average across batch sizes).}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Task \\ Domain
\end{tabular}} 
&
\multirow{2}{*}{
Model}
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Energy \\ (J)  
\end{tabular}} 
\\

&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{12}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification
\end{tabular}}
}
% 
& \multirow{2}{*}{
 Vt-b} &  1  & 2.3 \\ 
\cline{3-4}
 & &  8  & 2.6 \\ 
\cline{2-4}


% 
& \multirow{2}{*}
{Vt-l} & 1  & 2.5 \\ 
\cline{3-4}
 & &  8  & 6.7 \\ 
\cline{2-4}

%
& \multirow{2}{*}
{Vt-h}  & 1  & 4.4  \\ 
\cline{3-4}
& & 8  & 12.1 \\ 
\cline{2-4}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}} & 1 & 1.9 \\ 
\cline{3-4}
& & 8  & 2.6 \\ 
\cline{2-4}

% 
&\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}} & 1 & 3.6 \\ 
\cline{3-4}
% 
& &  8 & 4.8 \\ 
\cline{2-4}
% 

&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}}  & 1 & 3.9 \\ 
\cline{3-4}
& &  8 & 5.5 \\ 
\hline
% 
\multirow{6}{*}{Object Detection} 
&  \multirow{2}{*}{FRCNN}
& 1 & 3.5 \\ 
\cline{3-4}
%
& & 1 & 19.4 \\ 
\cline{2-4}
% 
&  \multirow{2}{*}{MRCNN}  & 1 & 3.6\\
\cline{3-4}
% 
& & 1 & 19.6\\
\cline{2-4}
% 

& \multirow{2}{*}{DETR} & 1 & 5.8 \\ 
\cline{3-4}
& & 8 & 23.1 \\ 
\hline
% 
\multirow{4}{*}{Image Segmenation} 
&  \multirow{2}{*}{MF}
& 1 & 11.4 \\ 
\cline{3-4}
%
& & 8 & 40.6 \\ 
\cline{2-4}
% 
&  \multirow{2}{*}{Seg}  & 1 & 1.7\\
\cline{3-4}
%
& & 8 & 4.6 \\ 
\hline
% 
\multirow{8}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 NLP \\  
\end{tabular}}} 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}} & 1 & 1.5 \\
\cline{3-4}
%
&& 8 & 1.5 \\
\cline{2-4}
% 
&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-L
\end{tabular}}}  & 1 & 5.1 \\
\cline{3-4}
%
& & 8 & 5.1 \\
\cline{2-4}
% 
&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & 11.1 \\
\cline{3-4}
%
& & 8 & 11.3 \\
\cline{2-4}
% 
& \multirow{2}{*}{Llama2} &   1 & 96.1 \\
\cline{3-4}
%
&  & 8 & 96.3 \\
\cline{2-4}
% 
&\multirow{2}{*} {bert} &   1 & 1.4 \\
\cline{3-4}
&  & 8 & 1.4 \\
\hline
%
\end{tabular}
\label{tab:energy}
\vspace{-4mm}
\end{table}
\end{center}

==> Tables/tab_expensive_ops.tex <==
\begin{center}
\begin{table}
\caption{\TODO{Update Task Domain Column}Most time-consuming non-GEMM operator groups for selected Models (Platform A, with GPU acceleration).}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Task \\ Domain
\end{tabular}} 
&
\multirow{2}{*}{
Model}
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification
\end{tabular}}
} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Vt-b    
\end{tabular}}
}  & 1 &  Norm  & 15 \\ 
\cline{3-5} 
% 
 & & 8 & Norm & 13  \\ 
\hline %\cline{2-5} 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} 
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-l 
\end{tabular}}} & 1 & Norm & 15 \\ 
\cline{3-5}
%
&& 8 & Norm & 12 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}}& 1 & Memory & 33.6 \\ 
\cline{3-5}
%
&& 8 & Memory & 30 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}}& 1 & Memory & 34 \\ 
\cline{3-5}
% 
 & & 8 & Memory & 31  \\
\hline
% 
 \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} &\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}} & 1 & Memory & 34 \\ 
\cline{3-5}
% 
&& 8 & Memory & 31 \\
\hline
%
\multirow{2}{*}{FasterRCNN} &  \multirow{2}{*}{FRCNN}& 1 & Memory & 38 \\ 
\cline{3-5}
%
&& 8 & Memory & 27 \\
\hline
%
 \multirow{2}{*}{MaskRCNN} &  \multirow{2}{*}{MRCNN} & 1 & Memory & 37\\
\cline{3-5}
%
&& 28 & Memory & 49 \\ 
\hline 
% 
 DETR & DETR & 1 & Norm & 34 \\ 
\hline 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}}& 1 & Act & 30 \\
\cline{3-5}
%
& &8 & Act & 30 \\ 
\hline
%
\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}}&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & Act & 28 \\
\cline{3-5}
%
&& 8 & Act & 28 \\ 
\hline
%
 Llama2-7B & Llama2& 1 &   Norm & 14 \\
\hline
%
\multirow{2}{*} {Bert} &\multirow{2}{*} {bert}& 1 &   Norm & 13 \\
\cline {3-5}
%
&& 8 &   Norm & 13 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_expensive_ops_old.tex <==
\begin{center}
\begin{table}
\caption{\bench Most Expensive NonGEMM Operator Group for selected \bench Models Running on Data Center GPU Platform.}

\scriptsize
\centering

\begin{tabular} {  |c | c | c | c | c |  } 
\hline

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Application  \\  
\end{tabular}} 
& 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Models  \\  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{9}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification 
\end{tabular}} 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Base 16  
\end{tabular}}
} & 1 & Norm  & 20 \\ 
\cline{3-5} 
% 
&  & 8 & Norm & 17  \\ 
\cline{2-5} 
%
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} & 1 & Norm & 20.5 \\ 
\cline{3-5}
%
&& 8 & Arith & 17 \\ 
\cline{2-5}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & 1 & Norm & 19 \\ 
\cline{3-5}
%
&& 8 & Norm & 18.5 \\ 
\cline {2-5}
% 
& \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} & 1 & Norm & 18 \\ 
\cline{3-5}
% 
& & 8 & Norm & 17  \\
\cline{2-5}
% 
& \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} & 1 & Norm & 18 \\ 
\cline{3-5}
% 
&& 8 & Norm & 18 \\
\hline
%
\multirow{7}{*}{Object Detection} & \multirow{3}{*}{FasterRCNN} & 1 & Norm & 60.5 \\ 
\cline{3-5}
%
&& 2 & Norm & 59 \\
\cline {3-5}
%
&& 8 & Norm & 49 \\
\cline {2-5}
%
& \multirow{3}{*}{MaskRCNN} & 1 & Norm & 58\\
\cline{3-5}
%
&& 2 & Norm & 56 \\ 
\cline {3-5}
% 
&& 8 & Norm & 49 \\ 
\cline {2-5}
% 
& DETR & 2 & Norm & 40 \\ 
\hline 
%
\multirow{7}{*}{Language Models} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 64 & Act & 16 \\ 
\cline {2-5}
%
& \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 64 & Act & 9 \\ 
\cline {2-5}
%
& Llama2-7B & 1 &   Arith & 23 \\
\cline {2-5}
%
&\multirow{2}{*} {Bert} & 1 &   Arith & 20 \\
\cline {3-5}
%
&& 64 &   Arith & 10 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_expensive_ops_shrinked.tex <==
\begin{center}
\begin{table}
\caption{Most Expensive non-GEMM Operator Group for selected Models Running on Data Center GPU Platform. \TODO{Update \% of exec time}}

\scriptsize
\centering

\begin{tabular} {   | c | c | c | c | c |  } 
\hline


\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Models  \\  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Model  \\ Alias  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Batch  \\ Size  
\end{tabular}} 
& 

\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
Operator  \\ Group  
\end{tabular}} 
&
\multirow{2}{*}{
\begin{tabular}[c]{@{}c@{}} 
\% of Exec.  \\ Time  
\end{tabular}} 
\\

&&&& \\

% \textbf{ Application } & \textbf{ Models } & \textbf{Batch} & \textbf{ Operator Group } & \textbf{\% of Exec.} 
%
%  &   &  \textbf{Size}& \textbf{Group }   & \textbf{Time }  \\
\hline
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Base 16  
\end{tabular}}
} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Vt-b    
\end{tabular}}
}  & 1 &  Norm  & 20 \\ 
\cline{3-5} 
% 
 & & 8 & Norm & 17  \\ 
\hline %\cline{2-5} 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 ViT  \\ Large 16  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Vt-l 
\end{tabular}}} & 1 & Norm & 20.5 \\ 
\cline{3-5}
%
&& 8 & Norm & 17 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Tiny  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Sw-t  
\end{tabular}}}& 1 & Memory & 19 \\ 
\cline{3-5}
%
&& 8 & Memory & 18.5 \\ 
\hline
% 
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Small  
\end{tabular}}} &\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
Sw-s  
\end{tabular}}}& 1 & Memory & 18 \\ 
\cline{3-5}
% 
 & & 8 & Memory & 17  \\
\hline
% 
 \multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 Swin  \\ Base   
\end{tabular}}} &\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
Sw-b   
\end{tabular}}} & 1 & Memory & 18 \\ 
\cline{3-5}
% 
&& 8 & Memory & 18 \\
\hline
%
\multirow{3}{*}{FasterRCNN} &  \multirow{3}{*}{FRCNN}& 1 & Memory & 60.5 \\ 
\cline{3-5}
%
& &2 & Memory & 59 \\
\cline {3-5}
%
&& 8 & Memory & 49 \\
\hline
%
 \multirow{3}{*}{MaskRCNN} &  \multirow{3}{*}{MRCNN} & 1 & Memory & 58\\
\cline{3-5}
%
&& 2 & Memory & 56 \\ 
\cline {3-5}
% 
&& 8 & Memory & 49 \\ 
\hline 
% 
 DETR & DETR & 1 & Norm & 40 \\ 
\hline 
%
\multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\  
\end{tabular}}} & \multirow{2}{*}{
{
\begin{tabular}[c]{@{}c@{}} 
gpt2  
\end{tabular}}}& 1 & Act & 23 \\
\cline{3-5}
%
& &8 & Act & 16 \\ 
\hline
%
\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
 GPT2  \\ X-Large 
\end{tabular}}}&\multirow{2}{*}{{
\begin{tabular}[c]{@{}c@{}} 
GPT2-XL
\end{tabular}}} & 1 & Act & 23 \\
\cline{3-5}
%
&& 8 & Act & 9 \\ 
\hline
%
 Llama2-7B & Llama2& 1 &   Norm & 23 \\
\hline
%
\multirow{2}{*} {Bert} &\multirow{2}{*} {bert}& 1 &   Norm & 20 \\
\cline {3-5}
%
&& 8 &   Norm & 10 \\ 
\hline

\end{tabular}
\label{tab:expensive_ops}

\end{table}
\end{center}

==> Tables/tab_microbench.tex <==
\begin{center}
\begin{table*}
\centering
\caption{A list of non-GEMM operators collected from eight popular model variants selected from Hugging Face listed in~\autoref{tab:modeltable}.\HK{I suggest to add one more column that shows the number of different input shapes/arguments in NonGEMM Bench} \RK{Add the characteristics of each operator}}
\scriptsize

\begin{tabular} {| c | c |  c | c | c |c| c | c| c|}
\hline 

\textbf{Operator Group}
% \multicolumn{1}{|c|}{\textbf{Operator Group}} 



& \multicolumn{1}{c|}{
\textbf{Operator}} 


& \multicolumn{1}{c|}{\textbf{Model}}


& \multicolumn{1}{c|}{\textbf{Single Operation}}


& \multicolumn{1}{c|}{\textbf{Single Operand}}


& \multicolumn{1}{c|}{\textbf{Non-Linearity}}


& \multicolumn{1}{c|}{\textbf{Dynamicity}}


& \multicolumn{1}{c|}{\textbf{Reduction}}



& \multicolumn{1}{c|}{\textbf{\# Input Shapes}} \\

\hline 

\multirow{4}{*}{Activation}
& ReLu 
& DETR
& \checkmark
& \checkmark
&  %checkmark
&  %\checkmark
&  %\checkmark
%Torch.nn.modules.activation
& \checkmark \\%\tiny [2,64,533],  \\
\cline{2-9} 

& GELU
& ViT-l16
%Torch.nn.modules.activation
& \checkmark
& \checkmark
& \checkmark
& 
& 
& \checkmark \\%\tiny [1, 97, 4096] \\
\cline{2-9}

& GELU 
& GPT2-XL 
%transformers.activations.GELUActivation
& \checkmark
& \checkmark
& \checkmark
&  
&  
& \checkmark \\%\tiny [1, 8, 6400] \\
\cline{2-9}

& SiLu 
& Llama-2 
& \checkmark %Torch.nn 
& \checkmark
& \checkmark
&  
& 
& \checkmark \\  %\tiny [1, 10, 11008]\\%, [1, 66, 11008], [1,338,11008] \\
\hline 


\multirow{6}{*}{Normalization}
& LayerNorm
& Segformer
&  %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 16384, 32]\\%, [2, 256, 32], [2, 4096, 64] \\
\cline{2-9} 

& BatchNorm2d
& Segformer
&   %Torch.nn.modules.batchnorm
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 256, 128, 128]\\% \\
\cline{2-9} 

& LlamaRMSNorm
& Llama
&  %transformers.models.llama
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 10, 4096]\\%, [1,338,4096], [1,118,4096]    \\ 
\cline{2-9} 

& FrozenBatchNorm2d
& MaskRCNN
&   %torchvision.ops.misc
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 1024, 50,68]\\%, [1, 256, 100, 136] \\
\cline{2-9} 

& FrozenBatchNorm2d
& DETR
&   %transformers.models.detr
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [2, 850, 256] \\
\cline{2-9} 

& LayerNorm
& DETR
&   %Torch.nn.modules.normalization
& \checkmark
& \checkmark
&  
& \checkmark

& \checkmark \\%\tiny [2, 850, 256]\\%, [2, 100, 256] \\
\hline 

\multirow{5}{*}{ Arithmetic} 
& Add
& Segformer
& \checkmark %Torch.add
&  
&  
&  
& 
& \checkmark \\%\tiny [2, 16384, 32]\\%, [2, 4096, 64], [2, 256, 256] \\
\cline{2-9} 

& Mul
& Llama-2
& \checkmark  %Torch.mul
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 10, 11008]\\%, [1, 66, 11008] \\ 
\cline{2-9} 

& Neg
& Llama-2
& \checkmark %Torch.neg
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 32, 10, 64] \\
\cline{2-9} 


& TrueDiv
& Segformer 

& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& \checkmark \\%\tiny [2, 1, 16384, 256]\\%, [2, 8, 256, 256] \\
\cline{2-9} 

& TrueDiv 
& GPT2-XL
& \checkmark %Torch.true\_divide
&  
&  
&  
&  
& \checkmark \\%\tiny [1, 25, 8, 8] \\
\hline 

% contiguous & Memory Op & Returns a new allocated tensor in a specified memory format \cite{paszke2019pytorch} & [391, 144, 4, 32] \\ 
% \hline 

% permute & Memory Op &  Returns a different view of the tensor based on the specified dimensions ~\cite{paszke2019pytorch} & [782, 144, 4, 32] \\ 
% \hline 

% view & Memory Op  & Allocates a new tensor in memory with same data as the input but with different shapes & [391, 12, 12, 1] \\ 
% \hline 


\multirow{9}{*}{Memory}  
& Contiguous
& Segformer
& \checkmark %Torch.Tensor.contiguous
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [2, 32, 128, 128]\\%, [2, 4096, 2, 32], [2, 64, 64, 64] \\
\cline{2-9} 

& Contiguous
& Llama-2
& \checkmark %Torch.Tensor
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 10, 32, 128]\\%, [1, 118, 32, 128] \\
\cline{2-9} 

& Permute
& ViT-b16
& \checkmark %Torch.permute
& \checkmark
&  
& 
&  
& \checkmark \\%\tiny [1, 768, 196]\\% \\ 
\cline{2-9} 

& Permute
& GPT2-XL
& \checkmark %Torch.permute
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 25, 64] \\
\cline{2-9} 

& Split
& GPT2-XL
& \checkmark %Torch.split
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 4800] \\ 
\cline{2-9} 

& View 
& GPT2-XL
& \checkmark %Torch.Tensor.view
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 8, 1600]\\
\cline{2-9} 

& Reshape
& ViT-b16
& \checkmark %Torch.reshape
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 768, 14, 14]\\
\cline{2-9} 

& Expand
& ViT-b16
& \checkmark %Torch.Tensor.expand
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 1, 768] \\
\cline{2-9} 

& Squeeze
& Llama-2
& \checkmark %Torch.squeeze
& \checkmark
&  
&  
&  
& \checkmark \\%\tiny [1, 1, 10, 128] \\ 
\hline 

%\multirow{2}{*}{Logit Computation} 
Logit 
& Softmax 
& DETR 
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
&  
& \checkmark
& \checkmark \\%\tiny [1, 25, 8, 8] \\ 
\cline{2-9} 

Computation
& Softmax
& Segformer
& \checkmark %Torch.nn.Functional.softmax
& \checkmark
& \checkmark
& 
& \checkmark
& \checkmark \\%\tiny [2, 1, 16384, 256]\\%, [2, 5, 1024, 256] \\ 
\hline 

RoI Selection
& NMS
& MaskRCNN
&  %torchvision.ops.nms
& 
& 
& \checkmark
& 
& \checkmark \\%\tiny [4663, 4] \\ 
\hline 

Interpolation
& Interpolate
& Segformer
&  %
& \checkmark
& 
& 
& 
& \checkmark \\%Torch.nn.Functional
%, [2, 256, 16, 16] \\
\hline 



\end {tabular}
\label{tab:microbench}
\end{table*}
\end{center}

==> Tables/tab_microbench_old.tex <==
\begin{center}
\begin{table}
\tiny
\begin{tabular} {| c | c |  c | c | c|}
\hline 
\textbf{Operator} & \textbf{Operator Group} & \textbf{Model} & \textbf{Implementation} & \textbf{Example Input Size} \\
\hline 

GELU & Activation & ViT-l16 & Torch.nn.modules.activation & [1, 97, 4096] \\
\hline

% GELU & Activation & Applies a custom implementation of gelu non linear activation function & [1, 8, 6400] \\
% \hline

% Softmax & Softmax & Applies a function to map the features/logits to probabilities & [1, 25, 8, 8] \\ 
% \hline 

% Tensor Addition & Arithmetic  & Performs an element wise addition on tensors & [[1, 12, 8, 8], [1, 1, 1, 8]] \\
% \hline

% TrueDiv & Arithmetic  & Performs an element wise division on tensors with rounding & [1, 32, 10, 10] \\ 
% \hline 

LlamaRMSNorm & Normalization & Llama & transformers.models.llama &  [1, 10, 4096], [1, 66, 4096], [1,338,4096], [1,118,4096]    \\ 
\hline 



FrozenBatchNorm2d & Normalization & MaskRCNN & torchvision.ops.misc  & [1, 1024, 50,68], [1, 512, 100, 136], [1, 256, 100, 136] \\
\hline 

Filter\_proposals & NMS & MaskRCNN & trochvisino.models.detection.rpn & [4663, 4] \\ 
\hline 

FrozenBatchNorm2d & Normalization & DETR & transformers.models.detr & [2, 850, 256] \\
\hline

% contiguous & Memory Op & Returns a new allocated tensor in a specified memory format \cite{paszke2019pytorch} & [391, 144, 4, 32] \\ 
% \hline 

% permute & Memory Op &  Returns a different view of the tensor based on the specified dimensions ~\cite{paszke2019pytorch} & [782, 144, 4, 32] \\ 
% \hline 

% view & Memory Op  & Allocates a new tensor in memory with same data as the input but with different shapes & [391, 12, 12, 1] \\ 
% \hline 

ReLu & Activation & DETR & Torch.nn.modules.activation &  [2,64,533],  \\
\hline 

LayerNorm & Normalization & DETR  & Torch.nn.modules.normalization & [2, 850, 256], [2, 100, 256] \\
\hline 

Softmax & Softmax & DETR & Torch.nn.Functional & [1, 25, 8, 8] \\ 
\hline 

LayerNorm & Normalization & Segformer  & Torch.nn.modules.normalization & [2, 16384, 32], [2, 256, 32], [2, 4096, 64], [2, 256, 64] \\
\hline 

BatchNorm2d & Normalization & Segformer & Torch.nn.modules.batchnorm & [2, 256, 128, 128] \\
\hline

contiguous & Memory Op & Segformer & Torch.Tensor & [2, 32, 128, 128], [2, 4096, 2, 32], [2, 64, 64, 64] \\
\hline 

Interpolate & Arithmetic & Segformer & Torch.nn.Functional & [2, 256, 128, 128], [2, 256, 64, 64], [2, 256, 32, 32], [2, 256, 16, 16] \\
\hline 

TrueDiv & Arithmetic & Segformer & Torch &  [2, 1, 16384, 256], [2, 2, 4096, 256], [2, 5, 1024, 256], [2, 8, 256, 256] \\
\hline 

Add & Arithmetic & Segformer & Torch & [2, 16384, 32], [2, 4096, 64], [2, 1024, 160], [2, 256, 256] \\
\hline 

Softmax & Softmax & Segformer & Torch.nn.Functional &  [2, 1, 16384, 256], [2, 2, 4096, 256], [2, 5, 1024, 256], [2, 8, 256, 256] \\ 
\hline 

SiLu & Activation & Llama-2 & Torch.nn &  [1, 10, 11008], [1, 66, 11008], [1,338,11008], [1,118,11008]\\
\hline 

mul & Arithmetic & Llama-2 & Torch &[1, 10, 11008], [1, 66, 11008] \\ 
\hline 

neg & Arithmetic & Llama-2 & Torch & [1, 32, 10, 64] \\
\hline 

contiguous & Memory Op & Llama-2 & Torch.Tensor & [1, 10, 32, 128], [1, 118, 32, 128] \\
\hline 

squeeze & Memory Op & Llama-2 & Torch &  [1, 1, 10, 128] \\ 
\hline 

GELU & Activation & GPT2-XL & transformers.activations & [1, 8, 6400] \\
\hline 

TrueDiv &Arithmetic& GPT2-XL & Torch & [1, 25, 8, 8] \\
\hline 

Split & Memory OP & GPT2-XL & Torch &[1, 8, 4800] \\ 
\hline 

view & Memory OP & GPT2-XL & Torch.Tensor & [1, 8, 1600]\\
\hline 

permute & Memory OP & GPT2-XL & Torch & [1, 8, 25, 64]\\
\hline 

reshape & Memory OP & ViT-b16 & Torch &  [1, 768, 14, 14]\\
\hline 

permute & Memory OP & ViT-b16 & Torch & [1, 768, 196] \\ 
\hline 

expand & Memory OP& ViT-b16 & Torch.Tensor & [1, 1, 768] \\
\hline 




\end {tabular}

\label{tab:microbench}
\caption{This table shows shows some of the NonGEMM operators collected while running \bench profiler. It categorizes each operator and provides input tensor size  examples.}
\end{table}
\end{center}

==> Tables/tab_model_table_fixed_old.tex <==
\begin{table}
    

\caption{\bench Tasks and Models. \HK{Please add references for each model and the dataset}}

\centering

\scriptsize
\begin{tabular} { |c|c|c|c|c |} 
\hline
%
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}c@{}} 
% Domain  \\  
% \end{tabular}} 
% & 

%
\textbf{ Domain }  & \textbf{ Application }  & \textbf{ Models }  & \textbf{ \# Params }  & \textbf{ Dataset } \\
\hline

\multirow{13}{*}{
\begin{tabular}[c]{@{}c@{}} 
Computer  \\ Vision 
\end{tabular}
} & \multirow{8}{*}{
\begin{tabular}[c]{@{}c@{}} 
Image  \\ Classification 
\end{tabular}
} & ResNet50~\cite{he2016deep} & 0.85M & ImageNet~\cite{imagenet_cvpr09} \\
\cline{3-5}
%
& & MobileNetv2~\cite{sandler2018mobilenetv2} & 3.4M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
%
&& ViT Base 16~\cite{kolesnikov2021ViT} & 86M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& ViT large 16~\cite{kolesnikov2021ViT}  & 307M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& ViT huge 14~\cite{kolesnikov2021ViT}  & 632M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5} 
% 
&& Swin tiny~\cite{liu2021swin} & 29M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5}
% 
&& Swin small~\cite{liu2021swin} & 50M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{3-5}
% 
&& Swin base~\cite{liu2021swin} & 88M & ImageNet~\cite{imagenet_cvpr09} \\ 
\cline{2-5}
% 
& \multirow{3}{*}{
\begin{tabular}[c]{@{}c@{}} 
Object \\ Detection 
\end{tabular} 
} & FasterRCNN~\cite{ren2015faster} & 42M & COCO~\cite{lin2014microsoft} \\ 
\cline{3-5}
&& MaskRCNN~\cite{he2017mask} & 44M & COCO~\cite{lin2014microsoft} \\
\cline{3-5}
%
&& DETR~\cite{carion2020end} & 41M & COCO~\cite{lin2014microsoft} \\ 
\cline{2-5}
%
&\multirow{2}{*}{Segmentation} & Maskformer~\cite{cheng2021per} & 102M & COCO~\cite{lin2014microsoft}\\
\cline{3-5}
%
&& SegFormer~\cite{xie2021segformer} & 3.7M & COCO~\cite{lin2014microsoft} \\
\hline
% 
\multirow{5}{*}{NLP} & \multirow{5}{*}{
\begin{tabular}[c]{@{}c@{}} 
Language  \\ Models 
\end{tabular} 
} & GPT2~\cite{achiam2023gpt} & 117M & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& GPT2 Large~\cite{achiam2023gpt} & 762M & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& GPT2 X-Large~\cite{achiam2023gpt} & 1.5B & wikitext~\cite{wikitext} \\
\cline{3-5}
%
&& Llama 2-7B~\cite{touvron2023llama} & 7B & wikitext~\cite{wikitext} \\
\cline {3-5}
%
&& Bert~\cite{kenton2019bert} & 110M & wikitext~\cite{wikitext} \\
\hline
\end{tabular}
\label{tab:modeltable}

\end{table}

==> Tables/tab_operator_group_summary.tex <==
\begin{center}
\begin{table}
\caption{Grouping non-GEMM operators based on Functionality}
\tiny
\begin{tabular} {| c | c | }
\hline 
\textbf{Operator Group} & \textbf{Description} \\
\hline 

Activation (Act) & Consists of linear and nonlinear activation functions  \\
\hline

Normalization (Norm)& Consists of different normalization functions \\
\hline

Softmax & Applies a function to map the features/logits to probabilities  \\ 
\hline 

Arithmetic (Arith) & Consists of operators performing element wise arithmetic operation on tensors\\
\hline

Memory Operations (MemOps) & Consists of operator performing allocating memory in different formats for tensors and returning different views and shapes of a tensor    \\ 
\hline 

NMS & Consists of non-maximum suppression functions used to filter out proposals \\ 

\hline 
%Embedding & Consists of the function performing the word and positional embedding in transformer based models\\  
%\hline 

\end {tabular}
\label{tab:operator_group_summary}
%\caption{Taxonomy for labeling and grouping NonGEMM operators.}

\end{table}
\end{center}
